Aplica\c{c}\~ao do Movimento Browniano Geom\'etrico para Simula\c{c}\~ao de Pre\c{c}os de A\c{c}\~oes do \'Indice Brasileiro de Small Caps

This work addressed the use of the geometric Brownian motion to simulate the prices of shares listed in the Small Caps index of the Brazilian stock exchange B3 (Brazil, Bolsa, Balc\~ao). The data used refer to the price history from January 2016 to December 2018. The price history of 2019 was used to be compared with the simulated prices. The data was imported from the Yahoo Finance database using the Python programming language, and the simulations were performed for each stock individually, and for portfolios formed based on expected returns, risk and the Sharpe Index. The results were better for portfolios with higher returns, lower risks and higher Sharpe Indexes.

==> 1-pre-textuais/errata.tex <==
\noindent FERRIGNO, C. R. A. \textbf{Tratamento de neoplasias ósseas apendiculares com reimplantação de enxerto ósseo autólogo autoclavado associado ao plasma rico em plaquetas}: estudo crítico na cirurgia de preservação de membro em cães. 2011. 128 f. Tese (Livre-Docência) - Faculdade de Medicina Veterinária e Zootecnia, Universidade de São Paulo, São Paulo, 2011.

\begin{table}[h!]
	\center
	\begin{tabular}{|p{1.4cm}|p{1cm}|p{3cm}|p{3cm}|}
		\hline
		\textbf{Folha} & \textbf{Linha} & \textbf{Onde se lê} &
		\textbf{Leia-se}\\
		\hline
		1 & 10 & auto-conclavo & autoconclavo\\
		\hline
	\end{tabular}
\end{table}


==> 1-pre-textuais/lista-de-abreviaturas-e-siglas.tex <==
\newacronym{ABNT}{ABNT}{Associação Brasileira de Normas Técnicas}
\newacronym{TEST}{TEST}{Tem que Escrever a Sigla no Texto }% use o comando \gls{} ao citar no texto para a sigla ficar visível na Lista. Caso a lista de abreviaturas não estiver aparecendo é porque você não utilizou o comando "gls" no texto. Exemplo no texto:   De acordo com o \gls{MCEG} ...  
\newacronym{PDF}{PDF}{\textit{Portable Document Format}}
\newacronym{MCEG}{MCEG}{modelo do circuito elétrico global}
\newacronym{CNTP}{CNTP}{condições normais de temperatura e pressão}
\newacronym{ELAT}{ELAT}{Grupo de Eletricidade Atmosférica}
\newacronym{INPE}{INPE}{Instituto Nacional de Pesquisas Espaciais}
\newacronym{DA}{DAs}{descargas atmosféricas}
\newacronym{SPDA}{SPDA}{Sistema de Proteção contra Descargas Atmosféricas}
\newacronym{TER}{TER}{técnica das esferas rolantes}
\newacronym{MPL}{MPL}{modelo da progressão do líder}
\newacronym{MEG}{MEG}{modelo eletrogeométrico}
\newacronym{TI}{TI}{temperatura de inversão}
\newacronym{SFW}{\textit{SFW}}{\textit{shilding failure width} / falha de blindagem}
\newacronym{LD}{\textit{LD}}{\textit{lateral distance}/distância lateral}



==> 1-pre-textuais/lista-de-simbolos.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%   Atencao! A lista nao ordena automaticamente   %%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{simbolos} \itemsep -1pt
	\item[$ Ae $] Área efetiva da antena
	\item[$ B $] Largura de faixa em que o ruído é medido em Hertz
	\item[$ d $] Distância em metros
	\item[$ E $] Campo elétrico
	\item[$ FA $] Fator da antena
	\item[$ Gr $] Ganho de recepção
	\item[$ h $] Altura efetiva ou comprimento efetivo de uma antena
	\item[$ I $] Corrente elétrica
	\item[$ k $] Constante de Boltzmann’s
	\item[$ K $] Eficiência de irradiação
	\item[$ M $] Variação do patamar de ruído em função da RBW
	\item[$ N $] Condutor de neutro
	\item[$ NF $] Figura de ruído
	\item[$ Ni $] Potência do ruído na entrada
	\item[$ No $] Potência do ruído na saída
	\item[$ P $] Potência
	\item[$ R $] Resistência
	\item[$ Si $] Potência do sinal na entrada
	\item[$ So $] Potência do sinal na saída
	\item[$ t $] Tempo
	\item[$ V $] Tensão
	\item[$ ZL  $] Impedância da antena
	\item[$ Zo $] Impedância de referência (50$\Omega$)
	\item[$ \lambda $] Comprimento de onda 
	\item[$ \Gamma $] Coeficiente de reflexão	
\end{simbolos}

==> Makefile <==
########################################################################
## Customizações do abnTeX2 (http://abnTeX2.googlecode.com)           ##
## para a Universidade Estadual do Ceara - UECE                       ##
##                                                                    ##
## This work may be distributed and/or modified under the             ## 
## conditions of the LaTeX Project Public License, either version 1.3 ##
## of this license or (at your option) any later version.             ##
## The latest version of this license is in                           ##
##   http://www.latex-project.org/lppl.txt                            ##
## and version 1.3 or later is part of all distributions of LaTeX     ##
## version 2005/12/01 or later.                                       ##
##                                                                    ##
## This work has the LPPL maintenance status `maintained'.            ##
##                                                                    ##
## The Current Maintainer of this work is Thiago Nascimento           ##
##                                                                    ##
## Project available on: https://github.com/thiagodnf/uecetex2        ##
##                                                                    ##
## Further information about abnTeX2                                  ##
## are available on http://abntex2.googlecode.com/                    ##
##                                                                    ##
########################################################################

filename=documento

all: compile
	
compile:
	@echo "*********************************************************"
	@echo "*                                                       *"
	@echo "* Package 'ueceTeX2' Release 1.0 -- 17 de Dezembro 2014 *"
	@echo "*                                                       *"
	@echo "*********************************************************"
	@echo "Compilando..."
	pdflatex $(filename).tex
	bibtex $(filename)
	makeglossaries $(filename)
	makeindex $(filename)
	pdflatex $(filename).tex
	pdflatex $(filename).tex
	@echo "Processo finalizado com sucesso!"

	
clean:
	@echo -n "Limpando arquivos auxiliares...\n"
	@rm -f *.out *.aux *.alg *.acr *.dvi *.gls *.log *.bbl *.blg *.ntn *.not *.lof *.lot *.toc *.loa *.lsg *.nlo *.nls *.ilg *.ind *.ist *.glg *.glo *.xdy *.acn *.idx *.loq *~
	@rm -f $(filename).pdf
	@echo "Processo finalizado com sucesso!"

